Watching ion-driven kinetics of ribozyme folding and misfolding caused by energetic and topological frustration one molecule at a time

Folding of ribozymes into well-defined tertiary structures usually requires divalent cations. How Mg$^{2+}$ ions direct the folding kinetics has been a long-standing unsolved problem because experiments cannot detect the positions and dynamics of ions. To address this problem, we used molecular simulations to dissect the folding kinetics of the Azoarcus ribozyme by monitoring the path each molecule takes to reach the folded state. We quantitatively establish that Mg$^{2+}$ binding to specific sites, coupled with counter-ion release of monovalent cations, stimulate the formation of secondary and tertiary structures, leading to diverse pathways that include direct rapid folding and trapping in misfolded structures. In some molecules, key tertiary structural elements form when Mg$^{2+}$ ions bind to specific RNA sites at the earliest stages of the folding, leading to specific collapse and rapid folding. In others, the formation of non-native base pairs, whose rearrangement is needed to reach the folded state, is the rate-limiting step. Escape from energetic traps, driven by thermal fluctuations, occurs readily. In contrast, the transition to the native state from long-lived topologically trapped native-like metastable states is extremely slow. Specific collapse and formation of energetically or topologically frustrated states occur early in the assembly process.

==> xx.tex <==
\relax 
\citation{HeilmanMillerI01JMB,Grilley06PNAS,Koculi07JACS,Bowman12COSB,Lipfert14ARBiochem,Sun17ARBiophys,Thirumalai05Biochem}
\citation{Pan97JMB,Roca18PNAS}
\citation{Xie04P}
\newlabel{FirstPage}{{}{1}{}{}{}}
\@writefile{toc}{\contentsline {title}{Watching ion-driven kinetics of ribozyme folding and misfolding caused by energetic and topological frustration one molecule at a time}{1}{}}
\citation{VicensCech06}
\citation{AzoXray04N}
\citation{Woodson10ARBiophys,Roh10JACS}
\citation{Rook99PNAS,Thirumalai00RNA}
\citation{Roh10JACS}
\citation{Chauhan08JACS}
\citation{Sinan11JBC}
\@writefile{toc}{\contentsline {abstract}{Abstract}{2}{}}
\@writefile{toc}{\contentsline {section}{\numberline {}Introduction}{2}{}}
\citation{Denesyuk15NatChem}
\citation{Denesyuk15NatChem,Hori19BJ}
\citation{Denesyuk15NatChem}
\citation{Hyeon05P}
\citation{Denesyuk13JPCB}
\citation{Denesyuk15NatChem}
\citation{Hori21PNAS}
\citation{AzoXray04N}
\citation{Honeycutt92}
\citation{Ermak78JCP}
\@writefile{toc}{\contentsline {section}{\numberline {}Materials and Methods}{4}{}}
\citation{Denesyuk15NatChem}
\citation{Roh10JACS}
\citation{DRID}
\citation{Denesyuk15NatChem}
\citation{Cate96S,Balasubramanian98P,Ding12NatMeth}
\citation{FreeSASA16}
\citation{Balasubramanian98P}
\citation{Adams04RNA}
\citation{TIS2AA,Humphris12JMB}
\citation{Amber16}
\citation{AzoXray04N}
\citation{Roh10JACS}
\citation{AzoXray04N}
\citation{Roh10JACS}
\citation{Behrouzi12Cell}
\citation{Behrouzi12Cell}
\@writefile{toc}{\contentsline {section}{\numberline {}Results}{6}{}}
\@writefile{lof}{\contentsline {figure}{\numberline {1}{\ignorespaces   \textbf  {Structure and Mg\textsuperscript  {2+}{}-mediated collapse of the \textit  {Azoarcus}{} ribozyme.} \textbf  {(a)} The secondary structure map shows that several helices are ordered along the sequence. The helices of the \textit  {Azoarcus}{} ribozyme are conventionally denoted as P2 through P9 (labeled in black). P2, P5, P6, P8, and P9 are hairpin structures in which adjacent segments form the double strands, whereas P3, P4, and P7 are double strands formed by non-local pairs of segments. Several key elements involving tertiary interactions are shown in red: TH, triple helix; SE, stack exchange; G site, Guanosine-binding site; TL2-TR8, tetraloop 2 and tetraloop-receptor 8; TL9-TR5, tetraloop 9 and tetraloop-receptor 5; and AS, the active site. \textbf  {(b)} Tertiary structure, taken from PDB 1U6B \citep  {AzoXray04N}. The same colors are used as in (a). \textbf  {(c)} Time dependence of the radius of gyration (\ensuremath  {R_{\textrm  {g}}}{}) averaged over 95 trajectories (thick red line). Thin lines show individual trajectories. At the beginning of the simulations $t=0$, the average \ensuremath  {R_{\textrm  {g}}}{} is $\ensuremath  {\left .\langle R_{\textrm  {g}} \rangle \right .}{}\approx $\nobreakspace  {}7.8\nobreakspace  {}nm, corresponding to the value at equilibrium in the absence of Mg\textsuperscript  {2+}{}. The fit using three exponential functions (see the main text) is shown by the blue dotted line. Inset: Coefficient of variation (C.V.), calculated as $\sqrt  {\left <\ensuremath  {R_{\textrm  {g}}}{}(t)^2\right >-\left <\ensuremath  {R_{\textrm  {g}}}{}(t)\right >^2}/\left <\ensuremath  {R_{\textrm  {g}}}{}(t)\right >$ where $\left <\right >$ is the average over the trajectories. \textbf  {(d)} The middle to late stages of compaction are magnified from the data in (c). The three time constants are indicated by blue vertical lines. \textbf  {(e)} Distance distribution functions reveal the stages in the collapse kinetics. The distribution functions were calculated using snapshots from the 95 trajectories at $t=0$, 0.15, 5, and 30 ms. The dotted lines are experimental tSAXS data from Ref.\nobreakspace  {}\citep  {Roh10JACS}. }}{7}{}}
\newlabel{fig:Fig1}{{1}{7}{}{}{}}
\citation{Roh10JACS}
\@writefile{lof}{\contentsline {figure}{\numberline {2}{\ignorespaces  \textbf  {Kinetic partitioning of the trajectories.} The blue and red arrows show the fate of the 95 folding trajectories initiated from the unfolded state (top left). The numbers beside the arrows indicate the fraction of trajectories in different pathways. In the compact structural ensemble, several representative misfolded structures, obtained from a clustering analysis, are shown. The structures labeled 'Misfold (P2)' (shown in the middle of the panel in the box) and 'Misfold (J8/7)' (lower left) are topological traps. Within the simulation time, 58\% of the trajectories reached the folded (native) state (right bottom), whereas 15\% were topologically trapped in the J8/7 misfolded state (left bottom). The remaining trajectories (27\%) are trapped in the compact-structure ensemble, partly because helices are mispaired (energetic trap). }}{8}{}}
\newlabel{fig:Fig2}{{2}{8}{}{}{}}
\citation{Roh10JACS}
\citation{Roh10JACS}
\citation{Roh10JACS}
\citation{Roh10JACS}
\newlabel{eq:Rg(t)}{{1}{9}{}{}{}}
\citation{Roh10JACS}
\citation{Guo95BP}
\citation{Brion97ARBiophys,Tinoco99JMB}
\@writefile{lof}{\contentsline {figure}{\numberline {3}{\ignorespaces   \textbf  {A representative rapid folding trajectory.} The ribozyme folds in $t\sim 2.4\,\textrm  {ms}$ without being kinetically trapped. \textbf  {(a)} Time dependent changes in $R_{g}$. \textbf  {(b-d)} Fraction of helix formations for (b) P3, (c) P6, and (d)P7. \textbf  {(e-j)} Fraction of major tertiary interactions (e) TL2-TR8, (f) TL9-TR5, (g) Triple Helix, (h) Stack Exchange, (i) G site, and (j) Active Site. See Fig.\nobreakspace  {}1{}{}{}\hbox {}(a-b) for the locations of these structural elements. Thin lines, with light colors are raw data, and thick lines with dark colors are averaged over 50 $\mu $s window. \textbf  {(Bottom)} Eight representative structures at several different time points. Major conformational changes are indicated by blue circles with labels. See Supplementary Movie 1 to watch the trajectory. }}{12}{}}
\newlabel{fig:Fig3}{{3}{12}{}{}{}}
\@writefile{lof}{\contentsline {figure}{\numberline {4}{\ignorespaces   \textbf  {Propensity to fold correctly is determined early.} \textbf  {(a)} A representative misfolding trajectory showing the formation of long-lived topologically-trapped states. Two key interactions in the peripheral regions, TL2-TR8 and TL9-TR5, formed early in the folding process ($t < 1$ ms), resulting in the junction J8/7 with an incorrect topology (See Fig.\nobreakspace  {}7{}{}{}\hbox {}). Because the incorrect chain topology cannot be resolved unless both of the peripheral interactions unfold, the RNA stays topologically trapped for the rest of the simulation time. See Fig.\nobreakspace  {}S14 for trajectories of \ensuremath  {R_{\textrm  {g}}}{}, fractions of secondary and tertiary elements, Fig.\nobreakspace  {}S15 for another example of a kinetic trap, and Supplementary Movie 2 for watching the trajectory. \textbf  {(b)} Specific collapse leads to rapid folding. From the distributions of the first passage times to the folded state, $P_{FP}^{F}(\tau _{F})$, we calculated, $\Phi ^F(t) = \DOTSI \intop \ilimits@ _{0}^{t}{P_{FP}^{F}(s)ds}$. Similarly, $\Phi ^M(t) = \DOTSI \intop \ilimits@ _{0}^{t}{P_{FP}^{M}(s)ds}$, where $P_{FP}^{M}$ is the distribution of mean first passage times to the trapped state. \textbf  {(c)} Fate of the ribozyme immediately following the initial collapse. The probability distributions of the structure overlap ($\chi $) with respect to the native structure; $\chi =0$ indicates no similarity to the crystal structure, and $\chi =1$ corresponds to the native state. (Inset) The distribution of $\chi $ immediately after collapse ($t < 150$ $\mu $s, green line, "Just-collapsed") compared with distributions of the equilibrium unfolded state (blue, [Mg\textsuperscript  {2+}] = 0 mM) and folded state (orange, [Mg\textsuperscript  {2+}] = 5 mM). The distribution of the "just-collapsed" ensemble in the main figure is decomposed into four distributions depending on the fate of each trajectory: Folded rapidly, trajectories reached the correct folded state within 5 ms; Folded slowly, trajectories reached the correct folded state after 5 ms but within the maximum simulation time (30 ms); Trapped, trajectories where the RNA was trapped in the major misfolded state; trajectories labeled Other were neither folded nor misfolded. }}{13}{}}
\newlabel{fig:Fig4}{{4}{13}{}{}{}}
\citation{Denesyuk15NatChem}
\citation{Denesyuk15NatChem}
\@writefile{lof}{\contentsline {figure}{\numberline {5}{\ignorespaces   \textbf  {Hierarchical formation of secondary and tertiary structures.} (a-d) Time-dependent formation of structural elements represented by the potential energies associated with (a) secondary hydrogen bond (H-bond), (b) secondary stacking, (c) tertiary H-bond, and (d) tertiary stacking. The thin lines are the results for the 95 individual trajectories, and the thick line in each panel is the average over all trajectories. (e) Time dependence of helix formation for helices P2 to P9. (f) Formation of six key elements associated with tertiary interactions (see Fig.\nobreakspace  {}1{}{}{}\hbox {}). }}{14}{}}
\newlabel{fig:Fig5}{{5}{14}{}{}{}}
\citation{Karplus76Nature}
\citation{HeilmanMillerI01JMB,Hori19BJ}
\citation{Oosawa71Book}
\citation{Hyeon12NatChem}
\citation{Kowerko15PNAS}
\citation{AzoXray04N}
\citation{Denesyuk15NatChem}
\citation{AzoXray04N}
\citation{Denesyuk15NatChem}
\citation{AzoXray04N}
\citation{AzoXray04N}
\@writefile{lof}{\contentsline {figure}{\numberline {6}{\ignorespaces   \textbf  {Fingerprints of Mg\textsuperscript  {2+}{} association and correlation with tertiary contact formation.} \textbf  {(a)} Number of cations condensed onto the RNA averaged over all the trajectories. At $t=0$, on average, there are 40 K\textsuperscript  {+}{} ions in the neighborhood of the ribozyme. K\textsuperscript  {+}{} cations are rapidly replaced by Mg\textsuperscript  {2+}{} in $t\apprle 0.02\,\textrm  {ms}$. \textbf  {(b-d)} Mg\textsuperscript  {2+}{} fingerprints, measured using local nucleotide-specific concentration at (b) $t=0.15$ ms, (c) 1.6 ms, and (d) 30 ms. Symbols indicate nucleotides that are either in direct contact with Mg\textsuperscript  {2+}{} (green circles) or linked via a water molecule (cyan squares) in the crystal structure \citep  {AzoXray04N}. The red crosses are nucleotides predicted to bind Mg\textsuperscript  {2+}{} in the equilibrium simulations \citep  {Denesyuk15NatChem}. \textbf  {(e)} Binding rates calculated from the mean first passage times of Mg\textsuperscript  {2+}{} binding event at each nucleotide. \textbf  {(f, g)} Trajectories displaying contact Mg\textsuperscript  {2+}{} concentration at nucleotides (f) A127 and (g) G130 taken from the folding trajectory shown in Fig.\nobreakspace  {}3{}{}{}\hbox {}. The folding times of the G site and Triple Helix (TH) are indicated by black arrows. \textbf  {(h)} A snapshot, at $t=0.11$ ms, when the G site is formed in the trajectory in (f) and (g). Nucleotides A127 and G130 are shown in stick, and Mg\textsuperscript  {2+}{} ions are spheres in red. \textbf  {(i, j)} Scatter plots of the first passage times of Mg\textsuperscript  {2+}{} binding to (i) A127 and (j) G130 versus the first passage time of the G site formation. If the Mg\textsuperscript  {2+}{} binding and the G site formation occurred concurrently ($|\tau _{\textrm  {G}} - \tau _i| < 0.2$ ms), the two events are regarded as strongly correlated and plotted in red; otherwise it is shown in blue. In each panel, the fraction of strong correlations (red points) is indicated by the percentage in red, associated with the Pearson correlation ($\rho $) calculated using all the data points. \textbf  {(k, l)} Same as (i-j) except for Mg\textsuperscript  {2+}{} binding to (k) U51 and (l) U126 versus the first passage time of Triple Helix (TH) formation. }}{16}{}}
\newlabel{fig:Fig6}{{6}{16}{}{}{}}
\citation{Denesyuk15NatChem}
\citation{AzoXray04N}
\citation{Denesyuk15NatChem}
\citation{Denesyuk15NatChem}
\citation{AzoXray04N}
\citation{Denesyuk15NatChem}
\citation{Su21Nature}
\citation{Bonilla22SciAdv}
\citation{Li22PNAS}
\citation{Adams04RNA,Rangan03PNAS,Chauhan08JACS}
\citation{Su21Nature}
\citation{Bonilla22SciAdv}
\citation{Li22PNAS}
\citation{Adams04RNA,Rangan03PNAS,Chauhan08JACS}
\citation{Cate96S,Balasubramanian98P,Ding12NatMeth}
\citation{Adams04RNA,Rangan03PNAS,Rangan03JMB,Rangan04JMB,Chauhan08JACS,Chauhan09JMB,Duncan10PLoSOne,Mitra11RNA}
\@writefile{lof}{\contentsline {figure}{\numberline {7}{\ignorespaces   \textbf  {Topological frustration in the persistent metastable state.} \textbf  {(a-c)} The major misfolded structure (J8/7) and its intermediate (b) are compared with the native intermediate and the folded structures (a). The spatial arrangements of J8/7 and other strands at the core are depicted on the right in blue and red circles. In the misfolding intermediate (b, left), the strand J8/7 (colored in red) passes through an incorrect location relative to the other two strands of the P3 helix (cyan), resulting in a topologically trapped state. This incorrect topology cannot be resolved unless other tertiary contacts such as TL2-TR8 (contact between domains P2 (orange) and P8 (blue)) disengage, which is unlikely to occur under the folding condition. As a consequence, it leads to a metastable state that is as compact as the folded state but with an incorrect chain topology. In panel (c), the same region in the native (upper, PDB 7EZ0 \cite  {Su21Nature}) and misfolded (lower, PDB 7UVT \cite  {Bonilla22SciAdv} and PDB 7XSK \cite  {Li22PNAS}) \textit  {Tetrahymena}{} ribozyme, solved by cryo-EM are shown for comparison. \textbf  {(d)} Comparison of experimental footprinting data with SASAs calculated from simulations. Protection factor ($F_{p}$) are calculated for the native (middle, blue) and misfolded ensembles (bottom, red) from simulations. Protected nucleotides, indicated by green-filled rectangles on top, are from data in three experiments, as labeled on the right \citep  {Adams04RNA,Rangan03PNAS,Chauhan08JACS}. The secondary structure is shown on top for reference. Note that protections of nucleotides in the P2 helix were not resolved in two experiments for technical reasons. }}{19}{}}
\newlabel{fig:Fig7}{{7}{19}{}{}{}}
\citation{Guo95BP,Thirumalai96AccChemRes}
\citation{Adams04RNA,Rangan03PNAS,Chauhan08JACS}
\citation{Chauhan08JACS}
\citation{Roh10JACS}
\citation{Koculi06JMB}
\citation{Guo95BP,Thirumalai01AnnuRevPhysChem}
\citation{Thirumalai01AnnuRevPhysChem}
\citation{Thirumalai95JdePhysique}
\citation{Hyeon12BJ}
\@writefile{toc}{\contentsline {section}{\numberline {}Discussion}{21}{}}
\citation{Garmann15RNA}
\citation{WuTinoco98PNAS}
\citation{Zarrinkar94Sci}
\citation{Wan10JMB}
\citation{Pan98JMB}
\citation{Pan00JMB}
\citation{Zhang05RNA}
\citation{Chauhan09JMB,Roh10JACS,Sinan11JBC}
\citation{Pan97JMB,Pan97NSB}
\citation{Sinan11JBC}
\citation{Russell06JMB}
\citation{Bonilla22SciAdv,Li22PNAS}
\citation{Perez-Salas04Biochemistry}
\citation{Rangan03JMB}
\citation{Perez-Salas04Biochemistry}
\citation{Rissone22PNAS,Bizarro12NAR}
\bibdata{AzoKineticsNotes,AzoKinetics}
\bibcite{HeilmanMillerI01JMB}{{1}{}{{}}{{}}}
\bibcite{Grilley06PNAS}{{2}{}{{}}{{}}}
\bibcite{Koculi07JACS}{{3}{}{{}}{{}}}
\bibcite{Bowman12COSB}{{4}{}{{}}{{}}}
\bibcite{Lipfert14ARBiochem}{{5}{}{{}}{{}}}
\bibcite{Sun17ARBiophys}{{6}{}{{}}{{}}}
\bibcite{Thirumalai05Biochem}{{7}{}{{}}{{}}}
\bibcite{Pan97JMB}{{8}{}{{}}{{}}}
\bibcite{Roca18PNAS}{{9}{}{{}}{{}}}
\bibcite{Xie04P}{{10}{}{{}}{{}}}
\bibcite{VicensCech06}{{11}{}{{}}{{}}}
\@writefile{toc}{\contentsline {section}{\numberline {}Acknowledgments}{24}{}}
\@writefile{toc}{\contentsline {section}{\numberline {}References}{24}{}}
\bibcite{AzoXray04N}{{12}{}{{}}{{}}}
\bibcite{Woodson10ARBiophys}{{13}{}{{}}{{}}}
\bibcite{Roh10JACS}{{14}{}{{}}{{}}}
\bibcite{Rook99PNAS}{{15}{}{{}}{{}}}
\bibcite{Thirumalai00RNA}{{16}{}{{}}{{}}}
\bibcite{Chauhan08JACS}{{17}{}{{}}{{}}}
\bibcite{Sinan11JBC}{{18}{}{{}}{{}}}
\bibcite{Denesyuk15NatChem}{{19}{}{{}}{{}}}
\bibcite{Hori19BJ}{{20}{}{{}}{{}}}
\bibcite{Hyeon05P}{{21}{}{{}}{{}}}
\bibcite{Denesyuk13JPCB}{{22}{}{{}}{{}}}
\bibcite{Hori21PNAS}{{23}{}{{}}{{}}}
\bibcite{Honeycutt92}{{24}{}{{}}{{}}}
\bibcite{Ermak78JCP}{{25}{}{{}}{{}}}
\bibcite{DRID}{{26}{}{{}}{{}}}
\bibcite{Cate96S}{{27}{}{{}}{{}}}
\bibcite{Balasubramanian98P}{{28}{}{{}}{{}}}
\bibcite{Ding12NatMeth}{{29}{}{{}}{{}}}
\bibcite{FreeSASA16}{{30}{}{{}}{{}}}
\bibcite{Adams04RNA}{{31}{}{{}}{{}}}
\bibcite{TIS2AA}{{32}{}{{}}{{}}}
\bibcite{Humphris12JMB}{{33}{}{{}}{{}}}
\bibcite{Amber16}{{34}{}{{}}{{}}}
\bibcite{Behrouzi12Cell}{{35}{}{{}}{{}}}
\bibcite{Guo95BP}{{36}{}{{}}{{}}}
\bibcite{Brion97ARBiophys}{{37}{}{{}}{{}}}
\bibcite{Tinoco99JMB}{{38}{}{{}}{{}}}
\bibcite{Karplus76Nature}{{39}{}{{}}{{}}}
\bibcite{Oosawa71Book}{{40}{}{{}}{{}}}
\bibcite{Hyeon12NatChem}{{41}{}{{}}{{}}}
\bibcite{Kowerko15PNAS}{{42}{}{{}}{{}}}
\bibcite{Su21Nature}{{43}{}{{}}{{}}}
\bibcite{Bonilla22SciAdv}{{44}{}{{}}{{}}}
\bibcite{Li22PNAS}{{45}{}{{}}{{}}}
\bibcite{Rangan03PNAS}{{46}{}{{}}{{}}}
\bibcite{Rangan03JMB}{{47}{}{{}}{{}}}
\bibcite{Rangan04JMB}{{48}{}{{}}{{}}}
\bibcite{Chauhan09JMB}{{49}{}{{}}{{}}}
\bibcite{Duncan10PLoSOne}{{50}{}{{}}{{}}}
\bibcite{Mitra11RNA}{{51}{}{{}}{{}}}
\bibcite{Thirumalai96AccChemRes}{{52}{}{{}}{{}}}
\bibcite{Koculi06JMB}{{53}{}{{}}{{}}}
\bibcite{Thirumalai01AnnuRevPhysChem}{{54}{}{{}}{{}}}
\bibcite{Thirumalai95JdePhysique}{{55}{}{{}}{{}}}
\bibcite{Hyeon12BJ}{{56}{}{{}}{{}}}
\bibcite{Garmann15RNA}{{57}{}{{}}{{}}}
\bibcite{WuTinoco98PNAS}{{58}{}{{}}{{}}}
\bibcite{Zarrinkar94Sci}{{59}{}{{}}{{}}}
\bibcite{Wan10JMB}{{60}{}{{}}{{}}}
\bibcite{Pan98JMB}{{61}{}{{}}{{}}}
\bibcite{Pan00JMB}{{62}{}{{}}{{}}}
\bibcite{Zhang05RNA}{{63}{}{{}}{{}}}
\bibcite{Pan97NSB}{{64}{}{{}}{{}}}
\bibcite{Russell06JMB}{{65}{}{{}}{{}}}
\bibcite{Perez-Salas04Biochemistry}{{66}{}{{}}{{}}}
\bibcite{Rissone22PNAS}{{67}{}{{}}{{}}}
\bibcite{Bizarro12NAR}{{68}{}{{}}{{}}}
\bibstyle{nar}
\providecommand\NAT@force@numbers{}\NAT@force@numbers
\newlabel{LastBibItem}{{68}{28}{}{}{}}
\newlabel{LastPage}{{}{28}{}{}{}}
\gdef \@abspage@last{28}

